Social-Media Activity Forecasting with Exogenous Information Signals

Due to their widespread adoption, social media platforms present an ideal environment for studying and understanding social behavior, especially on information spread. Modeling social media activity has numerous practical implications such as supporting efforts to analyze strategic information operations, designing intervention techniques to mitigate disinformation, or delivering critical information during disaster relief operations. In this paper we propose a modeling technique that forecasts topic-specific daily volume of social media activities by using both exogenous signals, such as news or armed conflicts records, and endogenous data from the social media platform we model. Empirical evaluations with real datasets from two different platforms and two different contexts each composed of multiple interrelated topics demonstrate the effectiveness of our solution.

==> sections/old_results.tex <==
\ignore{
\begin{figure*}[htpb]
\centering
\begin{tabular}{ccc}
	\subfloat[international/aid (VZ Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/international-aid_twitter_vz_cp1_shares.pdf}
			\label{fig:international-aid_twitter_vz}
	}
	&
\subfloat[maduro/legitimate (VZ Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/maduro-legitimate_twitter_vz_cp1_shares.pdf}
			\label{fig:maduro-legitimate_twitter_vz}
	}
	&
\subfloat[other/chavez (VZ Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/other-chavez_twitter_vz_cp1_shares.pdf}
			\label{fig:other-chavez_twitter_vz}
	}
\\
	\subfloat[maduro/cuba\_support (VZ YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/maduro-cuba_support_youtube_vz_cp1_shares.pdf}
			\label{fig:maduro-cuba-support_yt_vz}
	}
	&
\subfloat[military/desertions (VZ YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/military-desertions_youtube_vz_cp1_shares.pdf}
			\label{fig:military-desertions_yt_vz}
	}
	&
\subfloat[protests (VZ YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/protests_youtube_vz_cp1_shares.pdf}
			\label{fig:protests_yt_vz}
	}
\\
	\subfloat[leadership/sharif (CPEC Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/leadership-sharif_twitter_cpec_cp1_shares.pdf}
			\label{fig:leadership-sharif_twitter_cpec}
	}
	&
\subfloat[controversies/pakistan/baloch (CPEC Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/controversies-pakistan-baloch_twitter_cpec_cp1_shares.pdf}
			\label{fig:controversies-pakistan-baloch_twitter_cpec}
	}
	&
\subfloat[controversies/pakistan/students (CPEC Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/controversies-pakistan-students_twitter_cpec_cp1_shares.pdf}
			\label{fig:controversies-pakistan-students_twitter_cpec}
	}
\\
	\subfloat[benefits/development/roads (CPEC YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/benefits-development-roads_youtube_cpec_cp1_shares.pdf}
			\label{fig:benefits-development-roads_yt_cpec}
	}
	&
\subfloat[leadership/sharif (CPEC YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/leadership-sharif_youtube_cpec_cp1_shares.pdf}
			\label{fig:leadership-sharif_yt_cpec}
	}
	&
\subfloat[leadership/bajwa (CPEC YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/leadership-bajwa_youtube_cpec_cp1_shares.pdf}
			\label{fig:leadership-bajwa_yt_cpec}
	}
\\
\end{tabular}
	 \caption{Sample plots of Twitter and YouTube predictions for number of shares across two different contexts. Black line - ground truth, red line - MCAS predictions, green line - persistent baseline activity, and blue line - Hawkes predictions.}
	 \label{fig:sample_timeseries}
\end{figure*}
}


% Number of shares APE per topic performance
\begin{table*}[htpb]
\centering
\caption{Topic-wise APE performance on number of shares for our MCAS models and various baselines. The results presented are from the Twitter platform across two different datasets. Topics are ranked from most active to least active based on number of activities. Cells are bold if MCAS model outperforms all baselines.}
\label{tab:shares_ape_topic_performance}
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{Venezuela} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{protests} & \textbf{military} & \textbf{violence} & \textbf{guaido/legitimate} & \textbf{maduro/dictator} & \multicolumn{1}{c|}{\textbf{other/chavez}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 156.38 & \textbf{93.57} & 140.24 & 150.34 & \textbf{42.33} & \multicolumn{1}{c|}{37.18} \\
\multicolumn{1}{|l|}{MCAS-Int} & 127.43 & \textbf{77.55} & 160.96 & 93.70 & \textbf{48.61} & \multicolumn{1}{c|}{79.26} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 110.95 & \textbf{49.20} & 91.42 & 80.53 & \textbf{59.66} & \multicolumn{1}{c|}{51.49} \\
\multicolumn{1}{|l|}{ARIMA} & 89.62 & 195.65 & 56.46 & 69.56 & 100.43 & \multicolumn{1}{c|}{26.72} \\
\multicolumn{1}{|l|}{Hawkes} & 300.40 & 116.50 & 129.83 & 25.95 & 68.65 & \multicolumn{1}{c|}{84.25} \\
\multicolumn{1}{|l|}{Persistent} & 861.74 & 117.24 & 376.25 & 285.30 & 257.75 & \multicolumn{1}{c|}{377.64} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{arrests} & \textbf{international/aid} & \textbf{\begin{tabular}[c]{@{}c@{}}international/\\ respect\_sovereignty\end{tabular}} & \textbf{arrests/opposition} & \textbf{maduro/legitimate} & \multicolumn{1}{c|}{\textbf{other/chavez/anti}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & \textbf{84.18} & 106.86 & 94.40 & 39.79 & \textbf{117.25} & \multicolumn{1}{c|}{37.37} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{106.45} & 92.31 & 109.65 & 102.11 & 166.27 & \multicolumn{1}{c|}{\textbf{34.09}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{35.60} & \textbf{86.61} & 71.95 & 48.93 & \textbf{98.06} & \multicolumn{1}{c|}{48.22} \\
\multicolumn{1}{|l|}{ARIMA} & 117.56 & 150.67 & 144.97 & 38.71 & 214.47 & \multicolumn{1}{c|}{35.44} \\
\multicolumn{1}{|l|}{Hawkes} & 139.18 & 108.75 & 82.12 & 213.92 & 147.92 & \multicolumn{1}{c|}{50.88} \\
\multicolumn{1}{|l|}{Persistent} & 294.54 & 89.66 & 60.80 & 476.01 & 295.96 & \multicolumn{1}{c|}{226.93} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}other/\\ anti\_socialism\end{tabular}} & \textbf{maduro/narco} & \textbf{military/desertions} & \textbf{\begin{tabular}[c]{@{}c@{}}international/\\ aid\_rejected\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}maduro/\\ cuba\_support\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}other/\\ censorship\_outage\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 92.38 & \textbf{61.01} & 77.94 & 338.46 & \textbf{51.74} & \multicolumn{1}{c|}{\textbf{269.09}} \\
\multicolumn{1}{|l|}{MCAS-Int} & 83.57 & \textbf{65.96} & \textbf{43.25} & 201.09 & \textbf{55.23} & \multicolumn{1}{c|}{\textbf{283.14}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 41.59 & \textbf{52.95} & 74.89 & 153.01 & \textbf{95.83} & \multicolumn{1}{c|}{366.91} \\
\multicolumn{1}{|l|}{ARIMA} & 29.27 & 89.95 & 819.41 & 705.76 & 166.50 & \multicolumn{1}{c|}{2398.57} \\
\multicolumn{1}{|l|}{Hawkes} & 54.60 & 70.40 & 66.22 & 68.63 & 157.90 & \multicolumn{1}{c|}{359.67} \\
\multicolumn{1}{|l|}{Persistent} & 150.00 & 169.73 & 405.07 & 70.02 & 200.62 & \multicolumn{1}{c|}{2467.49} \\ \hline
\multicolumn{1}{c}{} &  &  & \textbf{} &  &  &  \\ \hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{CPEC} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{other} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/border\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/baloch\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}opposition/\\ propaganda\end{tabular}} & \textbf{leadership/sharif} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ roads\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 59.17 & \textbf{74.91} & 91.43 & \textbf{44.02} & 71.86 & \multicolumn{1}{c|}{\textbf{37.19}} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{17.13} & 263.78 & 92.40 & \textbf{53.53} & \textbf{33.49} & \multicolumn{1}{c|}{61.40} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 25.51 & 509.94 & 89.81 & \textbf{78.90} & \textbf{23.51} & \multicolumn{1}{c|}{53.21} \\
\multicolumn{1}{|l|}{ARIMA} & 64.67 & 115.22 & 101.70 & 89.36 & 53.19 & \multicolumn{1}{c|}{100.78} \\
\multicolumn{1}{|l|}{Hawkes} & 22.73 & 607.06 & 82.70 & 199.72 & 38.75 & \multicolumn{1}{c|}{47.32} \\
\multicolumn{1}{|l|}{Persistent} & 88.83 & 3616.17 & 236.36 & 468.44 & 188.90 & \multicolumn{1}{c|}{56.06} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ energy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/uighur\end{tabular}} & \textbf{benefits/jobs} & \textbf{leadership/bajwa} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/bajwa\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/students\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & \textbf{52.51} & \textbf{77.56} & \textbf{35.04} & 172.10 & 136.88 & \multicolumn{1}{c|}{\textbf{62.45}} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{57.11} & \textbf{41.09} & 61.40 & 105.19 & 346.38 & \multicolumn{1}{c|}{\textbf{95.65}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 70.26 & \textbf{93.07} & \textbf{33.88} & 113.16 & 191.27 & \multicolumn{1}{c|}{\textbf{472.68}} \\
\multicolumn{1}{|l|}{ARIMA} & 156.14 & 158.94 & 47.55 & 739.51 & 747.31 & \multicolumn{1}{c|}{468.82} \\
\multicolumn{1}{|l|}{Hawkes} & 57.17 & 106.70 & 100.48 & 144.18 & 246.21 & \multicolumn{1}{c|}{597.96} \\
\multicolumn{1}{|l|}{Persistent} & 80.19 & 309.21 & 50.68 & 91.70 & 65.39 & \multicolumn{1}{c|}{4651.04} \\ \hline
\end{tabular}
\end{table*}


\begin{table*}[htpb]
\centering
\caption{Topic-wise RMSE performance on number shares for our MCAS models and various baselines. The results presented are from the Twitter platform across two different datasets. Topics are ranked from most active to least active based on number of activities. Cells are bold if MCAS model outperforms all baselines.}
\label{tab:shares_rmse_topic_performance}
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{Venezuela} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{protests} & \textbf{military} & \textbf{violence} & \textbf{guaido/legitimate} & \textbf{maduro/dictator} & \multicolumn{1}{c|}{\textbf{other/chavez}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 39686.77 & \textbf{82475.95} & 64230.63 & 30527.90 & 16980.32 & \multicolumn{1}{c|}{13327.20} \\
\multicolumn{1}{|l|}{MCAS-Int} & 29659.20 & \textbf{69851.68} & 71043.76 & 24008.93 & \textbf{15676.03} & \multicolumn{1}{c|}{11989.04} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{26861.14} & \textbf{71387.17} & \textbf{54223.80} & 22053.58 & \textbf{15403.79} & \multicolumn{1}{c|}{10208.37} \\
\multicolumn{1}{|l|}{ARIMA} & 27822.29 & 90227.49 & 57414.61 & 21652.94 & 21512.57 & \multicolumn{1}{c|}{9076.91} \\
\multicolumn{1}{|l|}{Hawkes} & 45386.99 & 88491.17 & 58643.86 & 19641.50 & 16182.84 & \multicolumn{1}{c|}{11062.74} \\
\multicolumn{1}{|l|}{Persistent} & 145741.19 & 104836.70 & 85169.30 & 61052.77 & 39774.18 & \multicolumn{1}{c|}{47580.38} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{arrests} & \textbf{international/aid} & \textbf{\begin{tabular}[c]{@{}c@{}}international/\\ respect\_sovereignty\end{tabular}} & \textbf{arrests/opposition} & \textbf{maduro/legitimate} & \multicolumn{1}{c|}{\textbf{other/chavez/anti}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 8579.01 & \textbf{109673.50} & \textbf{32853.95} & 4493.59 & \textbf{9028.42} & \multicolumn{1}{c|}{4521.61} \\
\multicolumn{1}{|l|}{MCAS-Int} & 7533.87 & \textbf{100245.30} & \textbf{33892.89} & 4208.44 & 10296.12 & \multicolumn{1}{c|}{\textbf{3971.90}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{4680.99} & \textbf{105253.20} & \textbf{29849.80} & 3150.65 & \textbf{7902.81} & \multicolumn{1}{c|}{\textbf{4257.04}} \\
\multicolumn{1}{|l|}{ARIMA} & 7121.63 & 131401.43 & 36198.90 & 2592.57 & 10525.77 & \multicolumn{1}{c|}{4419.71} \\
\multicolumn{1}{|l|}{Hawkes} & 12733.79 & 120778.54 & 35792.56 & 9919.60 & 10253.41 & \multicolumn{1}{c|}{4697.53} \\
\multicolumn{1}{|l|}{Persistent} & 29685.89 & 118525.82 & 42859.05 & 27841.27 & 19359.05 & \multicolumn{1}{c|}{13284.31} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}other/\\ anti\_socialism\end{tabular}} & \textbf{maduro/narco} & \textbf{military/desertions} & \textbf{\begin{tabular}[c]{@{}c@{}}international/\\ aid\_rejected\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}maduro/\\ cuba\_support\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}other/\\ censorship\_outage\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 3666.36 & 5296.70 & 9205.26 & 26592.85 & \textbf{4191.62} & \multicolumn{1}{c|}{\textbf{8635.79}} \\
\multicolumn{1}{|l|}{MCAS-Int} & 2303.76 & 5059.26 & 9206.94 & 23608.35 & \textbf{4030.62} & \multicolumn{1}{c|}{9124.23} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{1564.03} & \textbf{4577.06} & 9508.23 & \textbf{21135.41} & \textbf{3827.76} & \multicolumn{1}{c|}{\textbf{8655.85}} \\
\multicolumn{1}{|l|}{ARIMA} & 2053.65 & 9954.98 & 18313.43 & 34615.19 & 6348.49 & \multicolumn{1}{c|}{14705.96} \\
\multicolumn{1}{|l|}{Hawkes} & 2111.73 & 4796.97 & 9145.85 & 21488.97 & 4379.73 & \multicolumn{1}{c|}{8904.02} \\
\multicolumn{1}{|l|}{Persistent} & 4988.26 & 6554.94 & 13624.04 & 21847.10 & 4565.25 & \multicolumn{1}{c|}{9134.22} \\ \hline
\multicolumn{1}{c}{} &  &  & \textbf{} &  &  &  \\ \hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{CPEC} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{other} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/border\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/baloch\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}opposition/\\ propaganda\end{tabular}} & \textbf{leadership/sharif} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ roads\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 16377.91 & \textbf{1460.22} & \textbf{926.60} & \textbf{495.29} & 1954.54 & \multicolumn{1}{c|}{2828.81} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{9412.69} & 2819.94 & \textbf{976.81} & \textbf{525.22} & \textbf{1442.12} & \multicolumn{1}{c|}{2653.42} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{11506.82} & 5791.20 & \textbf{935.46} & \textbf{541.76} & 1588.20 & \multicolumn{1}{c|}{2711.62} \\
\multicolumn{1}{|l|}{ARIMA} & 17392.51 & 1595.91 & 1042.04 & 646.05 & 1519.02 & \multicolumn{1}{c|}{2709.76} \\
\multicolumn{1}{|l|}{Hawkes} & 11761.90 & 5328.16 & 1091.68 & 1284.49 & 1761.78 & \multicolumn{1}{c|}{2461.50} \\
\multicolumn{1}{|l|}{Persistent} & 26499.10 & 63761.06 & 5807.37 & 3901.98 & 3189.86 & \multicolumn{1}{c|}{2878.01} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ energy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/uighur\end{tabular}} & \textbf{benefits/jobs} & \textbf{leadership/bajwa} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/bajwa\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/students\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 4423.58 & \textbf{3898.53} & \textbf{919.39} & 2469.30 & \textbf{991.76} & \multicolumn{1}{c|}{\textbf{40.78}} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{4229.84} & \textbf{4267.74} & 988.55 & \textbf{2353.44} & 1016.02 & \multicolumn{1}{c|}{\textbf{37.05}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{4057.32} & \textbf{4108.38} & \textbf{875.58} & \textbf{2317.22} & \textbf{897.33} & \multicolumn{1}{c|}{74.73} \\
\multicolumn{1}{|l|}{ARIMA} & 5441.25 & 5343.69 & 935.14 & 10973.03 & 1786.86 & \multicolumn{1}{c|}{74.03} \\
\multicolumn{1}{|l|}{Hawkes} & 4321.07 & 4338.48 & 1142.32 & 2381.76 & 1031.17 & \multicolumn{1}{c|}{113.06} \\
\multicolumn{1}{|l|}{Persistent} & 4949.80 & 5043.89 & 1166.93 & 2379.32 & 1013.00 & \multicolumn{1}{c|}{562.06} \\ \hline
\end{tabular}
\end{table*}


\begin{figure*}[htpb]
\centering
\begin{tabular}{ccc}
	\subfloat[arrests (VZ Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/arrests_twitter_vz_cp1_shares.pdf}
			\label{fig:arrests_twitter_vz}
	}
	&
\subfloat[maduro/legitimate (VZ Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/maduro-legitimate_twitter_vz_cp1_shares.pdf}
			\label{fig:maduro-legitimate_twitter_vz}
	}
	&
\subfloat[other/chavez (VZ Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/other-chavez_twitter_vz_cp1_shares.pdf}
			\label{fig:other-chavez_twitter_vz}
	}
\\
	\subfloat[maduro/cuba\_support (VZ YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/maduro-cuba_support_youtube_vz_cp1_shares.pdf}
			\label{fig:maduro-cuba-support_yt_vz}
	}
	&
\subfloat[military/desertions (VZ YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/military-desertions_youtube_vz_cp1_shares.pdf}
			\label{fig:military-desertions_yt_vz}
	}
	&
\subfloat[protests (VZ YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/protests_youtube_vz_cp1_shares.pdf}
			\label{fig:protests_yt_vz}
	}
\\
	\subfloat[benefits/jobs (CPEC Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/benefits-jobs_twitter_cpec_cp1_shares.pdf}
			\label{fig:benefits-jobs_twitter_cpec}
	}
	&
\subfloat[controversies/pakistan/baloch (CPEC Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/controversies-pakistan-baloch_twitter_cpec_cp1_shares.pdf}
			\label{fig:controversies-pakistan-baloch_twitter_cpec}
	}
	&
\subfloat[other (CPEC Twitter)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/other_twitter_cpec_cp1_shares.pdf}
			\label{fig:other_twitter_cpec}
	}
\\
	\subfloat[benefits/development/roads (CPEC YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/benefits-development-roads_youtube_cpec_cp1_shares.pdf}
			\label{fig:benefits-development-roads_yt_cpec}
	}
	&
\subfloat[leadership/sharif (CPEC YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/leadership-sharif_youtube_cpec_cp1_shares.pdf}
			\label{fig:leadership-sharif_yt_cpec}
	}
	&
\subfloat[other (CPEC YouTube)]{
		\includegraphics[width=0.28\linewidth]{images/timeseries_3week/other_youtube_cpec_cp1_shares.pdf}
			\label{fig:other-roads_yt_cpec}
	}
\\
\end{tabular}
	 \caption{Sample plots of Twitter and YouTube predictions for number of shares across two different scenarios. Black line - ground truth, red line - MCAS predictions, and green line - persistent baseline activity.}
	 \label{fig:sample_timeseries}
\end{figure*}


%%% Number of shares
\begin{table*}[htpb]
\centering
\caption{Topic-wise APE performance on number of shares for our MCAS models and various baselines. The results presented are from the Twitter platform across two different datasets.}
\label{tab:number_of_shares_topic_performance}
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{Venezuela} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{arrests} & \textbf{arrests/opposition} & \textbf{guaido/legitimate} & \textbf{international/aid} & \textbf{\begin{tabular}[c]{@{}c@{}}international/\\ aid\_rejected\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}international/\\ respect\_sovereignty\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & \textbf{84.18} & 39.79 & 150.34 & 106.86 & 338.46 & \multicolumn{1}{c|}{94.40} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{106.45} & 102.11 & 93.70 & 92.31 & 201.09 & \multicolumn{1}{c|}{109.65} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{35.60} & 48.93 & 80.53 & \textbf{86.61} & 153.01 & \multicolumn{1}{c|}{71.95} \\
\multicolumn{1}{|l|}{ARIMA} & 117.56 & 38.71 & 69.56 & 150.67 & 705.76 & \multicolumn{1}{c|}{144.97} \\
\multicolumn{1}{|l|}{Hawkes} & 139.18 & 213.92 & 25.95 & 108.75 & 68.63 & \multicolumn{1}{c|}{82.12} \\
\multicolumn{1}{|l|}{Persistent} & 294.54 & 476.01 & 285.30 & 89.66 & 70.02 & \multicolumn{1}{c|}{60.80} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}maduro/\\ cuba\_support\end{tabular}} & \textbf{maduro/dictator} & \textbf{maduro/legitimate} & \textbf{maduro/narco} & \textbf{military} & \multicolumn{1}{c|}{\textbf{military/desertions}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & \textbf{51.74} & \textbf{42.33} & \textbf{117.25} & \textbf{61.01} & \textbf{93.57} & \multicolumn{1}{c|}{77.94} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{55.23} & \textbf{48.61} & 166.27 & \textbf{65.96} & \textbf{77.55} & \multicolumn{1}{c|}{\textbf{43.25}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{95.83} & \textbf{59.66} & \textbf{98.06} & \textbf{52.95} & \textbf{49.20} & \multicolumn{1}{c|}{74.89} \\
\multicolumn{1}{|l|}{ARIMA} & 166.50 & 100.43 & 214.47 & 89.95 & 195.65 & \multicolumn{1}{c|}{819.41} \\
\multicolumn{1}{|l|}{Hawkes} & 157.90 & 68.65 & 147.92 & 70.40 & 116.50 & \multicolumn{1}{c|}{66.22} \\
\multicolumn{1}{|l|}{Persistent} & 200.62 & 257.75 & 295.96 & 169.73 & 117.24 & \multicolumn{1}{c|}{405.07} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}other/\\ anti\_socialism\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}other/\\ censorship\_outage\end{tabular}} & \textbf{other/chavez} & \textbf{other/chavez/anti} & \textbf{protests} & \multicolumn{1}{c|}{\textbf{violence}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 92.38 & \textbf{269.09} & 37.18 & 37.37 & 156.38 & \multicolumn{1}{c|}{140.24} \\
\multicolumn{1}{|l|}{MCAS-Int} & 83.57 & \textbf{283.14} & 79.26 & \textbf{34.09} & 127.43 & \multicolumn{1}{c|}{160.96} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 41.59 & 366.91 & 51.49 & 48.22 & 110.95 & \multicolumn{1}{c|}{91.42} \\
\multicolumn{1}{|l|}{ARIMA} & 29.27 & 2398.57 & 26.72 & 35.44 & 89.62 & \multicolumn{1}{c|}{56.46} \\
\multicolumn{1}{|l|}{Hawkes} & 54.60 & 359.67 & 84.25 & 50.88 & 300.40 & \multicolumn{1}{c|}{129.83} \\
\multicolumn{1}{|l|}{Persistent} & 150.00 & 2467.49 & 377.64 & 226.93 & 861.74 & \multicolumn{1}{c|}{376.25} \\ \hline
\multicolumn{1}{c}{} &  &  & \textbf{} &  &  &  \\ \hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{CPEC} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ energy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ roads\end{tabular}} & \textbf{benefits/jobs} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/border\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/uighur\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/bajwa\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & \textbf{52.51} & \textbf{37.19} & \textbf{35.04} & \textbf{74.91} & \textbf{77.56} & \multicolumn{1}{c|}{136.88} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{57.11} & 61.40 & 61.40 & 263.78 & \textbf{41.09} & \multicolumn{1}{c|}{346.38} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 70.26 & 53.21 & \textbf{33.88} & 509.94 & \textbf{93.07} & \multicolumn{1}{c|}{191.27} \\
\multicolumn{1}{|l|}{ARIMA} & 156.14 & 100.78 & 47.55 & 115.22 & 158.94 & \multicolumn{1}{c|}{747.31} \\
\multicolumn{1}{|l|}{Hawkes} & 57.17 & 47.32 & 100.48 & 607.06 & 106.70 & \multicolumn{1}{c|}{246.21} \\
\multicolumn{1}{|l|}{Persistent} & 80.19 & 56.06 & 50.68 & 3616.17 & 309.21 & \multicolumn{1}{c|}{65.39} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/baloch\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/students\end{tabular}} & \textbf{leadership/bajwa} & \textbf{leadership/sharif} & \textbf{\begin{tabular}[c]{@{}c@{}}opposition/\\ propaganda\end{tabular}} & \multicolumn{1}{c|}{\textbf{other}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 91.43 & \textbf{62.45} & 172.10 & 71.86 & \textbf{44.02} & \multicolumn{1}{c|}{59.17} \\
\multicolumn{1}{|l|}{MCAS-Int} & 92.40 & \textbf{95.65} & 105.19 & \textbf{33.49} & \textbf{53.53} & \multicolumn{1}{c|}{\textbf{17.13}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 89.81 & 472.68 & 113.16 & \textbf{23.51} & \textbf{78.90} & \multicolumn{1}{c|}{25.51} \\
\multicolumn{1}{|l|}{ARIMA} & 101.70 & 468.82 & 739.51 & 53.19 & 89.36 & \multicolumn{1}{c|}{64.67} \\
\multicolumn{1}{|l|}{Hawkes} & 82.70 & 597.96 & 144.18 & 38.75 & 199.72 & \multicolumn{1}{c|}{22.73} \\
\multicolumn{1}{|l|}{Persistent} & 236.36 & 4651.04 & 91.70 & 188.90 & 468.44 & \multicolumn{1}{c|}{88.83} \\ \hline
\end{tabular}
\end{table*}

%%%% Number of new users
\begin{table*}[htpb]
\centering
\caption{Topic-wise APE performance on number of new users for our MCAS models and various baselines. The results presented are from the Twitter platform across two different datasets.}
\label{tab:number_of_users_topic_performance}
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{Venezuela} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{arrests} & \textbf{arrests/opposition} & \textbf{guaido/legitimate} & \textbf{international/aid} & \textbf{\begin{tabular}[c]{@{}c@{}}international/\\ aid\_rejected\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}international/\\ respect\_sovereignty\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & \textbf{79.46} & \textbf{101.17} & \textbf{22.16} & \textbf{46.46} & 136.79 & \multicolumn{1}{c|}{\textbf{138.70}} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{24.87} & \textbf{109.36} & \textbf{110.90} & \textbf{123.96} & 261.09 & \multicolumn{1}{c|}{\textbf{85.40}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 212.34 & 226.04 & 265.10 & \textbf{203.31} & 174.55 & \multicolumn{1}{c|}{\textbf{95.24}} \\
\multicolumn{1}{|l|}{ARIMA} & 179.44 & 145.94 & 115.02 & 266.33 & 7409.53 & \multicolumn{1}{c|}{155.86} \\
\multicolumn{1}{|l|}{Persistent} & 776.77 & 995.09 & 852.87 & 291.92 & 124.04 & \multicolumn{1}{c|}{199.92} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}maduro/\\ cuba\_support\end{tabular}} & \textbf{maduro/dictator} & \textbf{maduro/legitimate} & \textbf{maduro/narco} & \textbf{military} & \multicolumn{1}{c|}{\textbf{military/desertions}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 124.06 & \textbf{60.79} & 166.70 & \textbf{38.66} & \textbf{100.61} & \multicolumn{1}{c|}{\textbf{79.19}} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{64.01} & \textbf{53.76} & 203.73 & \textbf{46.43} & \textbf{263.26} & \multicolumn{1}{c|}{\textbf{65.10}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 266.24 & 129.82 & 213.90 & \textbf{51.29} & \textbf{116.97} & \multicolumn{1}{c|}{\textbf{52.30}} \\
\multicolumn{1}{|l|}{ARIMA} & 119.56 & 128.74 & 133.93 & 196.50 & 311.27 & \multicolumn{1}{c|}{456.81} \\
\multicolumn{1}{|l|}{Persistent} & 431.34 & 653.15 & 783.29 & 206.63 & 305.56 & \multicolumn{1}{c|}{586.45} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}other/\\ anti\_socialism\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}other/\\ censorship\_outage\end{tabular}} & \textbf{other/chavez} & \textbf{other/chavez/anti} & \textbf{protests} & \multicolumn{1}{c|}{\textbf{violence}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 359.47 & \textbf{250.89} & \textbf{31.67} & \textbf{20.55} & \textbf{28.29} & \multicolumn{1}{c|}{169.78} \\
\multicolumn{1}{|l|}{MCAS-Int} & 225.97 & \textbf{164.55} & \textbf{51.06} & \textbf{32.81} & \textbf{71.46} & \multicolumn{1}{c|}{193.04} \\
\multicolumn{1}{|l|}{MCAS-Ens} & \textbf{116.94} & \textbf{584.62} & 83.39 & 77.07 & 158.72 & \multicolumn{1}{c|}{154.46} \\
\multicolumn{1}{|l|}{ARIMA} & 175.27 & 2548.24 & 77.99 & 68.80 & 77.32 & \multicolumn{1}{c|}{105.07} \\
\multicolumn{1}{|l|}{Persistent} & 315.41 & 5244.74 & 608.24 & 504.75 & 1328.79 & \multicolumn{1}{c|}{557.96} \\ \hline
\multicolumn{1}{c}{} &  &  & \textbf{} &  &  &  \\ \hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{CPEC} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ energy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}benefits/develop/\\ roads\end{tabular}} & \textbf{benefits/jobs} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/border\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ china/uighur\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/bajwa\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 154.92 & \textbf{149.84} & \textbf{76.17} & \textbf{78.53} & 1607.91 & \multicolumn{1}{c|}{81.60} \\
\multicolumn{1}{|l|}{MCAS-Int} & \textbf{59.48} & \textbf{120.16} & \textbf{65.14} & 188.73 & \textbf{58.13} & \multicolumn{1}{c|}{71.00} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 132.24 & \textbf{114.55} & 168.15 & 2751.40 & \textbf{223.86} & \multicolumn{1}{c|}{137.88} \\
\multicolumn{1}{|l|}{ARIMA} & 831.65 & 210.68 & 159.82 & 86.34 & 268.26 & \multicolumn{1}{c|}{430.40} \\
\multicolumn{1}{|l|}{Persistent} & 118.97 & 159.43 & 114.57 & 5573.29 & 342.05 & \multicolumn{1}{c|}{61.52} \\ \hline
\multicolumn{1}{|l|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/baloch\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}controversies/\\ pakistan/students\end{tabular}} & \textbf{leadership/bajwa} & \textbf{leadership/sharif} & \textbf{\begin{tabular}[c]{@{}c@{}}opposition/\\ propaganda\end{tabular}} & \multicolumn{1}{c|}{\textbf{other}} \\ \hline
\multicolumn{1}{|l|}{MCAS-Exo} & 524.79 & 1150.73 & \textbf{70.11} & 232.19 & \textbf{61.73} & \multicolumn{1}{c|}{\textbf{123.42}} \\
\multicolumn{1}{|l|}{MCAS-Int} & 87.59 & \textbf{154.04} & \textbf{55.85} & \textbf{35.94} & \textbf{74.38} & \multicolumn{1}{c|}{\textbf{76.76}} \\
\multicolumn{1}{|l|}{MCAS-Ens} & 177.07 & 454.57 & \textbf{79.66} & 128.86 & 582.20 & \multicolumn{1}{c|}{\textbf{106.93}} \\
\multicolumn{1}{|l|}{ARIMA} & 45.99 & 209.74 & 423.91 & 113.17 & 216.01 & \multicolumn{1}{c|}{126.40} \\
\multicolumn{1}{|l|}{Persistent} & 629.89 & 5502.05 & 97.07 & 296.88 & 915.25 & \multicolumn{1}{c|}{205.93} \\ \hline
\end{tabular}
\end{table*}

%%%% Number of new users avg.
\begin{table}[ht]
\centering
\caption{Evaluation of MCAS model variations and baselines for number of new users forecasting. The table presents the mean performance across various topics of interest in four different forecasting metrics. The performance for a given topic was averaged across the three weeks that were predicted. The forecasting periods are 2019-02-15 to 2019-03-07 for Venezuela and  2020-07-14 to 2020-08-03 for CPEC. Cells are bold if our MCAS model outperforms all baselines.}
\label{tab:new_users_performance}
\begin{tabular}{|c|c|r|r|r|r|}
\hline
\textbf{Domain} & \textbf{Model} & \multicolumn{1}{c|}{\textbf{APE}} & \multicolumn{1}{c|}{\textbf{SMAPE}} & \multicolumn{1}{c|}{\textbf{RMSE}} & \multicolumn{1}{c|}{\textbf{DTW}} \\ \hline
 & MCAS-Exo & \textbf{108.63} & \textbf{101.08} & \textbf{4104.19} & 0.85 \\
VZ & MCAS-Int & \textbf{119.49} & \textbf{90.91} & \textbf{4051.47} & 0.81 \\
Twitter & MCAS-Ens & \textbf{176.79} & \textbf{97.01} & \textbf{3934.68} & 0.73 \\
 & ARIMA & 703.98 & 116.76 & 7066.06 & 0.88 \\
 & Persistent & 820.38 & 105.33 & 9135.58 & 0.66 \\ \hline
 & MCAS-Exo & 64.82 & \textbf{70.88} & \textbf{125.21} & 0.89 \\
VZ & MCAS-Int & 75.45 & \textbf{72.02} & \textbf{125.14} & 0.88 \\
YouTube & MCAS-Ens & 56.44 & \textbf{61.35} & \textbf{117.11} & 0.93 \\
 & ARIMA & 70.92 & 87.19 & 145.29 & 0.81 \\
 & Persistent & 49.22 & 85.83 & 138.78 & 0.77 \\ \hline
 & MCAS-Exo & 359.33 & \textbf{109.91} & 1660.57 & 0.85 \\
CPEC & MCAS-Int & \textbf{87.27} & \textbf{97.88} & \textbf{1051.88} & \textbf{0.78} \\
Twitter & MCAS-Ens & 421.45 & \textbf{112.76} & 2426.61 & 0.81 \\
 & ARIMA & 260.20 & 124.24 & 1510.72 & 0.83 \\
 & Persistent & 1168.07 & 126.58 & 3808.78 & 0.80 \\ \hline
 & MCAS-Exo & \textbf{51.50} & \textbf{84.21} & 49.04 & \textbf{0.80} \\
CPEC & MCAS-Int & \textbf{64.81} & \textbf{77.93} & \textbf{41.63} & \textbf{0.79} \\
YouTube & MCAS-Ens & \textbf{47.94} & \textbf{72.31} & 48.38 & \textbf{0.78} \\
 & ARIMA & 104.31 & 85.84 & 47.05 & 0.86 \\
 & Persistent & 75.06 & 95.71 & 60.30 & 0.80 \\ \hline
\end{tabular}
\end{table}


% number of shares avg. performance
\begin{table}[ht]
\centering
\caption{Evaluation of MCAS model variations and baselines for number of shares forecasting. The table presents the mean performance across various topics of interest in four different forecasting metrics. The performance for a given topic was averaged across the three weeks that were predicted. The forecasting periods are 2019-02-15 to 2019-03-07 for Venezuela and  2020-07-14 to 2020-08-03 for CPEC. Cells are bold if our MCAS model outperforms all baselines.}
\label{tab:shares_performance}
\begin{tabular}{|c|c|r|r|r|r|}
\hline
\textbf{Domain} & \textbf{Model} & \multicolumn{1}{c|}{\textbf{APE}} & \multicolumn{1}{c|}{\textbf{SMAPE}} & \multicolumn{1}{c|}{\textbf{RMSE}} & \multicolumn{1}{c|}{\textbf{DTW}} \\ \hline
 & MCAS-Exo & \textbf{110.58} & 95.56 & \textbf{26331.52} & 0.89 \\
 & MCAS-Int & \textbf{107.26} & \textbf{88.26} & \textbf{24206.13} & 0.84 \\
VZ & MCAS-Ens & \textbf{89.88} & \textbf{78.68} & \textbf{22472.26} & 0.88 \\
Twitter & ARIMA & 302.76 & 101.63 & 28108.81 & 0.92 \\
 & Hawkes & 124.76 & 93.31 & 26911.77 & 0.81 \\
 & Persistent & 399.04 & 100.94 & 44245.76 & 0.69 \\ \hline
 & MCAS-Exo & 92.96 & \textbf{80.92} & 203.82 & 0.94 \\
 & MCAS-Int & 63.25 & \textbf{69.11} & \textbf{171.74} & 0.95 \\
VZ & MCAS-Ens & 58.76 & \textbf{66.75} & \textbf{165.57} & 0.90 \\
YouTube & ARIMA & 79.61 & 90.26 & 198.36 & 0.86 \\
 & Hawkes & 80.36 & 119.86 & 241.87 & 0.80 \\
 & Persistent & 51.73 & 89.42 & 186.65 & 0.78 \\ \hline
 & MCAS-Exo & \textbf{76.26} & \textbf{102.91} & \textbf{3065.56} & 0.82 \\
 & MCAS-Int & \textbf{102.38} & \textbf{99.62} & \textbf{2560.24} & 0.90 \\
CPEC & MCAS-Ens & \textbf{146.27} & \textbf{101.04} & \textbf{2950.47} & 0.85 \\
Twitter & ARIMA & 236.93 & 115.21 & 4121.61 & 0.86 \\
 & Hawkes & 187.58 & 103.99 & 3084.78 & 0.80 \\
 & Persistent & 825.25 & 121.18 & 10096.03 & 0.78 \\ \hline
 & MCAS-Exo & \textbf{51.38} & 83.61 & 122.62 & 0.82 \\
 & MCAS-Int & 53.16 & \textbf{69.54} & \textbf{114.10} & 0.81 \\
CPEC & MCAS-Ens & \textbf{50.13} & \textbf{78.65} & \textbf{116.03} & 0.80 \\
YouTube & ARIMA & 87.12 & 81.65 & 121.54 & 0.87 \\
 & Hawkes & 51.38 & 95.58 & 157.65 & 0.82 \\
 & Persistent & 66.55 & 95.00 & 143.66 & 0.77 \\ \hline
\end{tabular}
\end{table}

%%% Friedman statistical ranking
\begin{table}[htpb]
\centering
\caption{The average ranking scores across topics for each model. Friedman statistical test ranking in terms of APE and RMSE performance. The ranking scores for each model are defined by the average ranks across topics. Most ranking scores are statistically significant (significance level of 0.02) with the exception of YouTube shares in CPEC, and YouTube new users in both CPEC and VZ. This means we reject the null hypothesis which states that all the algorithms are equivalent and so their ranks.}
\label{tab:friedman_ranking_performance}
\begin{tabular}{|c|cc|cc|}
\hline
\textbf{Domain} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Rank \\ (Shares)\end{tabular}}} & \textbf{Model} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Rank \\ (New Users)\end{tabular}}} & \textbf{Model} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}VZ\\ Twitter\end{tabular}} & 1.61 & MCAS-Ens & 1.72 & MCAS-Int \\
 & 3.0 & MCAS-Int & 2.33 & MCAS-Ens \\
 & 3.38 & Hawkes & 2.77 & MCAS-Exo \\
 & 3.55 & MCAS-Exo & 3.44 & ARIMA \\
 & 3.94 & ARIMA & 4.72 & Persistent \\
 & 5.5 & Persistent & - & - \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}VZ\\ YouTube\end{tabular}} & 2.27 & MCAS-Ens & 2.05 & MCAS-Ens \\
 & 2.77 & MCAS-Exo & 2.94 & MCAS-Exo \\
 & 3.5 & Persistent & 3.11 & ARIMA \\
 & 3.55 & ARIMA & 3.33 & Hawkes \\
 & 4.0 & MCAS-Int & 3.55 & MCAS-Int \\
 & 4.88 & Hawkes & - & - \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}CPEC\\ Twitter\end{tabular}} & 2.33 & MCAS-Int & 1.41 & MCAS-Int \\
 & 2.41 & MCAS-Ens & 2.5 & MCAS-Ens \\
 & 2.75 & MCAS-Exo & 3.25 & MCAS-Exo \\
 & 4.0 & Hawkes & 3.33 & ARIMA \\
 & 4.16 & ARIMA & 4.5 & Persistent \\
 & 5.33 & Persistent & - & - \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}CPEC\\ YouTube\end{tabular}} & 2.0 & MCAS-Ens & 2.0 & MCAS-Ens \\
 & 2.7 & MCAS-Exo & 2.5 & MCAS-Exo \\
 & 3.6 & ARIMA & 3.2 & ARIMA \\
 & 3.9 & MCAS-Int & 3.3 & MCAS-Int \\
 & 4.2 & Hawkes & 4.0 & Persistent \\
 & 4.6 & Persistent & - & - \\ \hline
\end{tabular}
\end{table}
